Boundary corrections for kernel approximation to differential operators

Kernel-based approach to operator approximation for partial differential equations has been shown to be unconditionally stable for linear PDEs and numerically exhibit unconditional stability for non-linear PDEs. These methods have the same computational cost as an explicit finite difference scheme but can exhibit order reduction at boundaries. In previous work on periodic domains, [8,9], order reduction was addressed, yielding high-order accuracy. The issue addressed in this work is the elimination of order reduction of the kernel-based approach for a more general set of boundary conditions. Further, we consider the case of both first and second order operators. To demonstrate the theory, we provide not only the mathematical proofs but also experimental results by applying various boundary conditions to different types of equations. The results agree with the theory, demonstrating a systematic path to high order for kernel-based methods on bounded domains.

==> ch4modification_old.tex <==
\section{Generalized Kernel Based Schemes}

Now we need to make these operators to be high order but directly using these operator fails and modification is needed. Consider $k=2$ case:
	\begin{align*}
	\mathcal{D}_{L}[\phi](x)
	= - \frac{1}{\alpha}\phi'(x)- \frac{1}{\alpha^2}\phi''(x) + \frac{1}{\alpha^2}\phi''(b) e^{-\alpha(b-x)} - \frac{1}{\alpha^{3}}I_{L}[\phi'''](x).
	\end{align*}
Instead of adding successively defined term $\mathcal{D}_{L}^p=\mathcal{D}_{L}[\mathcal{D}_{L}^{p-1}]$, $p\geq 2$, we define
	$$ \mtD_{L}[\phi](x) :=\mathcal{D}_{L}[\phi](x) - \frac{1}{\alpha^2}\phi''(b) e^{-\alpha(b-x)} $$
and apply the $\mathcal{D}_L$ operator:
\begin{align*} %\widetilde
\mathcal{D}_L[\mtD_{L}[\phi]](x) = \frac{1}{\alpha^2}\phi''(x)+\frac{1}{\alpha^{3}}I_{L}[\phi'''](x)+\frac{1}{\alpha^{3}}I_{L}^2[\phi'''](x).
\end{align*}
Then we obtain higher order approximation to $\phi'(x)$ with the modified partial sum:
\begin{align*}
\mathcal{D}_L[\phi](x) + \mathcal{D}_L[\mtD_{L}[\phi]](x) - \frac{1}{\alpha^2}\phi''(b) e^{-\alpha(b-x)} = - \frac{1}{\alpha}\phi'(x) + \mathcal{O}(\frac{1}{\alpha^3}).
\end{align*}
We generalize this modification to get the higher order in the following.

\subsection{Modification of derivative operators}%\label{sec:modify}

Using the general boundary treatments, we can modify the partial sums for the first derivative operators.
\begin{subequations}\label{eq:mod_sum}
\begin{align} %\widetilde
\phi_{x}^{+}(x) &\approx {\mP}^{L}_{k}[\phi](x)=
-\alpha \left( \mD_{L}[\phi](x)+ \sum\limits_{p=2}^{k}\mtD_{L}^p[\phi](x) \right), \\
\phi_{x}^{-}(x) &\approx{\mP}^{R}_{k}[\phi](x)=
\alpha \left( \mD_{R}[\phi](x)+\sum\limits_{p=2}^{k}\mtD_{R}^p[\phi](x)  \right) \\
\phi_{xx}(x) &\approx{\mP}^{0}_{k}[\phi](x)=
-\alpha^2  \left( \mD_{0}[\phi](x)+\sum\limits_{p=2}^{k}\mtD_{0}^p[\phi](x) \right)
% \nonumber \\
% & \qquad \qquad \qquad  +\left(\frac{1}{\alpha}\right)^{4}\frac{\mu\partial_{x}^{4}v(a)-\partial_{x}^{4}v(b)}{1-\mu^2} e^{-\alpha(b-x)} + \left(\frac{1}{\alpha}\right)^{4}\frac{\mu\partial_{x}^{4}v(b)-\partial_{x}^{4}v(a)}{1-\mu^2} e^{-\alpha(x-a)} ) 
\label{eq:mod_sum_0}
\end{align}
\end{subequations}
where ${\mtD}_{L}$, ${\mtD}_{R}$ and ${\mtD}_{0}$ are given as
\begin{subequations}\label{eq:expression}
	\begin{align}
	& \left\{\begin{array}{ll}\label{eq:expressionL}
    \mttD_{L}[\phi](x) =\mD_{L}[\phi](x) +  \sum_{m=2}^{k} C(1,m) \left(\frac{1}{\alpha}\right)^{m}\partial_{x}^{m}\phi(b) e^{-\alpha(b-x)},\\
	\mttD_{L}^p[\phi](x) =\mtD_{L}^p[\phi](x) +  \sum_{m=p}^{k} C(p,m) \left(\frac{1}{\alpha}\right)^{m}\partial_{x}^{m}\phi(b) e^{-\alpha(b-x)}, \quad p\geq 2,\\
	\displaystyle \mtD_{L}^p[\phi](x) =\mathcal{D}_{L}[\mttD_{L}^{p-1}][\phi](x), \quad p\geq 2,\\
    C(1,m) = -1, C(p,m) = -\sum\limits_{i=p-1}^{m-1} C(p-1,i),
	\end{array}
	\right.\\
    & \left\{\begin{array}{ll}\label{eq:expressionR}
    \mttD_{R}[\phi](x) =\mD_{R}[\phi](x) +  \sum_{m=2}^{k} C(1,m) \left(-\frac{1}{\alpha}\right)^{m}\partial_{x}^{m}\phi(b) e^{-\alpha(x-a)},\\
	\mttD_{R}^p[\phi](x) =\mtD_{R}^p[\phi](x) +  \sum_{m=p}^{k} C(p,m) \left(-\frac{1}{\alpha}\right)^{m}\partial_{x}^{m}\phi(a) e^{-\alpha(x-a)},\quad p\geq 2,\\
	\displaystyle \mtD_{R}^p[\phi](x) =\mathcal{D}_{R}[\mttD_{R}^{p-1}][\phi](x), \quad p\geq 2,\\
    C(1,m) = -1, C(p,m) = -\sum\limits_{i=p-1}^{m-1} C(p-1,i),
	\end{array}
	\right.\\
    & \left\{\begin{array}{ll}\label{eq:expression0}
    % \mttD_{0}[\phi](x) = \mD_{0}[\phi](x) + \frac{1}{2}\sum\limits_{m=2}^{k} C(1,m) \left( (\frac{1}{\alpha})^{2m} \partial_{x}^{2m}\phi(a) + (-\frac{1}{\alpha})^{2m+1} \partial_{x}^{2m+1}\phi(a)\right) e^{-\alpha(x-a)}
    %   \\ 
    %   \qquad \qquad  \qquad \qquad \quad + \frac{1}{2} \sum\limits_{m=2}^{k} C(1,m) \left( (\frac{1}{\alpha})^{2m} \partial_{x}^{2m}\phi(b) + (\frac{1}{\alpha})^{2m+1} \partial_{x}^{2m+1}\phi(b)\right) e^{-\alpha(b-x)},\\
    % \mtD_{0}^1[\phi](x) = \mD_0 [\phi](x), \\
	\mttD_{0}^p[\phi](x) = \mtD_{0}^p[\phi](x) + \frac{1}{2}\sum\limits_{m=p+1}^{k} C(p,m-1) \left( (\frac{1}{\alpha})^{2m} \partial_{x}^{2m}\phi(a) + (-\frac{1}{\alpha})^{2m+1} \partial_{x}^{2m+1}\phi(a)\right) e^{-\alpha(x-a)}
      \\ 
      \qquad \qquad  \qquad \qquad \quad + \frac{1}{2} \sum\limits_{m=p+1}^{k} C(p,m-1) \left( (\frac{1}{\alpha})^{2m} \partial_{x}^{2m}\phi(b) + (\frac{1}{\alpha})^{2m+1} \partial_{x}^{2m+1}\phi(b)\right) e^{-\alpha(b-x)},\\
     \qquad \qquad  \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad p\geq 1,\\
	\displaystyle \mtD_{0}^p[\phi](x) =\mathcal{D}_{0}[\mttD_{0}^{p-1}][\phi](x), \quad p\geq 2,\\
    C(1,m) = -1, C(p,m) = -\sum\limits_{i=p-1}^{m-1} C(p-1,i),
	\end{array}
	\right.
 %    & \left\{\begin{array}{ll}\label{eq:expression0}
 %    \mttD_{0}[\phi](x) = \mD_{0}[\phi](x) - \sum_{m=2}^{k} C(1,m) \left(\frac{1}{\alpha}\right)^{2m}\left(\frac{\mu\partial_{x}^{2m}\phi(a)-\partial_{x}^{2m}\phi(b)}{1-\mu^2} e^{-\alpha(b-x)} +\frac{\mu\partial_{x}^{2m}\phi(b)-\partial_{x}^{2m}\phi(a)}{1-\mu^2} e^{-\alpha(x-a)}\right),\\
 %    % \mtD_{0}^1[\phi](x) = \mD_0 [\phi](x), \\
	% \mttD_{0}^p[\phi](x) =\mtD_{0}^p[\phi](x) -  \sum_{m=p}^{k} C(p,m) \left(\frac{1}{\alpha}\right)^{2m}\left(\frac{\mu\partial_{x}^{2m}\phi(a)-\partial_{x}^{2m}\phi(b)}{1-\mu^2} e^{-\alpha(b-x)} +\frac{\mu\partial_{x}^{2m}\phi(b)-\partial_{x}^{2m}\phi(a)}{1-\mu^2} e^{-\alpha(x-a)}\right), \\
 %     \qquad \qquad  \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad p\geq 2,\\
	% \displaystyle \mtD_{0}^p[\phi](x) =\mathcal{D}_{0}[\mttD_{0}^{p-1}][\phi](x), \quad p\geq 2,\\
 %    C(1,m) = -1, C(p,m) = -\sum\limits_{i=p-1}^{m-1} C(p-1,i),
	% \end{array}
	% \right.
	\end{align}
\end{subequations}
In developing the modified sums for these operators, we assume that the derivatives of $\phi$ have been constructed at the boundaries, i.e., $\partial_{x}^{m}\phi(a)$ and $\partial_{x}^{m}\phi(b)$, $m\geq1$. In practice, with inverse Lax-Wendroff (ILW) method, we could have odd-order, even-order or all the derivatives of $\phi$; see for example \cite[Section 2.2.3]{christlieb2019kernel}. So based on different information you have, you may need to adjust the general boundary operators. 


\subsection{Convergence analysis}%\label{sec:modify}
The modified partial sum \eqref{eq:mod_sum} is constructed so that it agrees with the derivative values at the boundary, to preserve consistency with the boundary condition imposed on $\phi$. 
To verify the accuracy of these modified sums, we start with following lemmas.
\begin{lemma}
    
\end{lemma}

\begin{thm}
 Suppose $\phi\in\mathcal{C}^{k+1}[a,b]$, $k=1, \, 2,\, 3$. Then, the modified partial sums \eqref{eq:mod_sum} satisfy
	\begin{align}
		 \|\partial_{x}\phi(x)-{\mP}^{*}_{k}[\phi](x)\|_{\infty}\leq C \left(\frac{1}{\alpha}\right)^{k} \|\partial_{x}^{k+1}\phi(x)\|_{\infty}
	\end{align}
	where $*$ indicates $L$ and $R$ operators.
 \end{thm}
\begin{proof}
It is obvious for the $k=1$ case from the partial sums \eqref{eq:sum} and Lemma \ref{lem_D}. We here consider left-sided first derivative approximations, ${\mP}^{L}_{k}[\phi]$, for $k\geq 2$ cases. We first give another equivalent definition of $\mtD_{L}^{p}[\phi](x)$ for $2 \le p \le k$ as the follows. 
  \begin{align}\label{eqn:DtLAnotherform}
	 \mtD_{L}^{p}[\phi](x) = & \sum_{m=p}^{k}C(p,m)\left(\frac{1}{\alpha}\right)^{m} \left(\partial^{m}_{x}\phi(x) -\partial_{x}^{m}\phi(b) e^{-\alpha(b-x)} \right) \nonumber\\
 & + (-1)^p (\frac{1}{\alpha})^{k+1}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m+1)|(I_L)^m[\partial_{x}^{k+1}\phi](x).
\end{align}
  When $p = 2$, \eqref{eqn:DtLAnotherform} is same as what we get from \eqref{eq:expressionL}. In fact, with \eqref{eqn:DtLAnotherform}, we have
	\begin{align*}
	\mttD_{L}[\phi](x) =\mtD_{L}[\phi](x) -  \sum_{m=2}^{k}\left(\frac{1}{\alpha}\right)^{m}\partial_{x}^{m}\phi(b) e^{-\alpha(b-x)}
	\end{align*}
	and then we can differentiate it,
	\begin{align*}
	\begin{split}
		\partial_{x}\mttD_L[\phi](x) &= \partial_{x} \left( -\sum_{p=1}^{k} \left(\frac{1}{\alpha}\right)^{p}\partial_{x}^{p}\phi(x) -\left(\frac{1}{\alpha}\right)^{k+1}I_{L}[\partial_{x}^{k+1}\phi](x) \right) \\
		&=	-\sum_{p=1}^{k} \frac{1}{\alpha^{p}}\partial_{x}^{p+1}\phi(x)- \frac{1}{\alpha^{k+1}}\partial_{x}I_L[\partial_{x}^{k+1}\phi](x) \\
		&= 	-\sum_{p=1}^{k-1} \frac{1}{\alpha^{p}}\partial_{x}^{p+1}\phi(x)- \frac{1}{\alpha^{k}}I_L[\partial_{x}^{k+1}\phi](x),
	\end{split}
	\end{align*}
	by using Lemma \ref{lem_D}. Repeating the above process, we can find a general form for $0\leq \ell \leq k$,
	\begin{align*}
		\partial_{x}^{\ell}\mttD_L[\phi](x) = -\sum_{p=1+\ell}^{k} \frac{1}{\alpha^{p-\ell}}\partial_{x}^{p}\phi(x)- \frac{1}{\alpha^{k+1-\ell}}I_L[\partial_{x}^{k+1}\phi](x).
	\end{align*}
	Now again from the equation in Lemma \ref{lem_D} with using $k-1$-th sum instead of $k$-th sum, we apply the operator $\mD_L$ to $\mttD_{L}[\phi]$:
        \begin{align*}
	\mtD_{L}^{2}[\phi](x) & =\mathcal{D}_{L}[\mttD_{L}^{1}][\phi](x)  \\
 & = \sum_{p=2}^{k}(p-1)\left(\frac{1}{\alpha}\right)^{p} \left(\partial^{p}_{x}\phi(x) -\partial_{x}^{p}\phi(b) e^{-\alpha(b-x)} \right) + (\frac{1}{\alpha})^{k+1} I_L[I_L[\partial_{x}^{k+1}\phi]](x) + (k-1) (\frac{1}{\alpha})^{k+1}I_L[\partial_{x}^{k+1}\phi](x),
	\end{align*}
 which is same as \eqref{eqn:DtLAnotherform} with $p = 2$. 
% 	Therefore, 
% 	\begin{align*}
% 	\mD_L[\phi](x)+\mtD_{L}^{2}[\phi](x)= -\frac{1}{\alpha}\partial_{x} \phi(x) +
%    \sum_{p=2}^{k}(p-2)\left(\frac{1}{\alpha}\right)^{p} \left(\partial^{p}_{x}\phi(x) -\partial_{x}^{p}\phi(b) e^{-\alpha(b-x)} \right) \\
% + (\frac{1}{\alpha})^{k+1} I_L[I_L[\partial_{x}^{k+1}\phi]](x) + (k-2) (\frac{1}{\alpha})^{k+1}I_L[\partial_{x}^{k+1}\phi](x),
% 	\end{align*}
 Now we prove $p > 2$ cases by induction. Assume that for $p \ge 2$, \eqref{eqn:DtLAnotherform} is equivalent from the definition of \eqref{eq:expressionL}, then we consider $p+1$ case. Since
 \begin{align*}
	\mttD_{L}^{p}[\phi](x)  = & \sum_{m=p}^{k}C(p,m)\left(\frac{1}{\alpha}\right)^{m} \partial^{m}_{x}\phi(x)+(-1)^p (\frac{1}{\alpha})^{k+1}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m+1)|(I_L)^m[\partial_{x}^{k+1}\phi](x), 
	\end{align*}
 and then we can differentiate it,
 \begin{align*}
	\begin{split}
		\partial_{x}\mttD_{L}^{p}[\phi](x) &= \partial_{x} \left( \sum_{m=p}^{k}C(p,m)\left(\frac{1}{\alpha}\right)^{m} \partial^{m}_{x}\phi(x)+(-1)^p (\frac{1}{\alpha})^{k+1}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m+1)|(I_L)^m[\partial_{x}^{k+1}\phi](x) \right) \\
		&= \sum_{m=p}^{k}C(p,m)\left(\frac{1}{\alpha}\right)^{m} \partial^{m+1}_{x}\phi(x)+(-1)^p (\frac{1}{\alpha})^{k+1}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m+1)|\partial_{x}(I_L)^m[\partial_{x}^{k+1}\phi](x)  \\
		&= \sum_{m=p}^{k}C(p,m)\left(\frac{1}{\alpha}\right)^{m} \partial^{m+1}_{x}\phi(x)+ (-1)^p (\frac{1}{\alpha})^{k} |C(p,m)|(I_L[\partial_{x}^{k+1}\phi](x) - \partial_{x}^{k+1}\phi) \\
        & \quad + (-1)^p (\frac{1}{\alpha})^{k}  \sum\limits_{m = 2}^{p} |C(p-m+1,k-m+1)|\left((I_L)^m[\partial_{x}^{k+1}\phi](x) - (I_L)^{m-1}[\partial_{x}^{k+1}\phi](x)\right) \\ 
        &= \sum_{m=p}^{k-1}C(p,m)\left(\frac{1}{\alpha}\right)^{m} \partial^{m+1}_{x}\phi(x) + (-1)^p (\frac{1}{\alpha})^{k} (I_L)^p [\partial_{x}^{k+1}\phi](x) \\
        & \quad + (-1)^p (\frac{1}{\alpha})^{k}  \sum\limits_{m = 1}^{p-1} \left(|C(p-m+1,k-m+1) + C(p-m,k-m)|\right)(I_L)^m[\partial_{x}^{k+1}\phi](x) \\
        &= \sum_{m=p}^{k-1}C(p,m)\left(\frac{1}{\alpha}\right)^{m} \partial^{m+1}_{x}\phi(x) + (-1)^p (\frac{1}{\alpha})^{k}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m)|(I_L)^m[\partial_{x}^{k+1}\phi](x),
	\end{split}
	\end{align*}
    where note that if $p$ is even, $|C(p,m)| = C(p,m)$ and if $p$ is odd, $|C(p,m)| = -C(p,m)$. Note that $C(p,m-1) = C(p,m) + C(p-1,m-1)$ and repeating the above process, we can find a general form for $0 \leq \ell \leq k+1-p$,we have   
    \begin{align*}
	\begin{split}
		\partial_{x}^l \mttD_{L}^{p}[\phi](x) &= \sum_{m=p}^{k-\ell}C(p,m)\left(\frac{1}{\alpha}\right)^{m} \partial^{m+\ell}_{x}\phi(x) \\  
         & \quad + (-1)^p (\frac{1}{\alpha})^{k-\ell+1}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m-\ell+1)|(I_L)^m[\partial_{x}^{k+1}\phi](x) \\
         & = \sum_{m=p+\ell}^{k}C(p,m-\ell)\left(\frac{1}{\alpha}\right)^{m-\ell} \partial^{m}_{x}\phi(x) \\  
         & \quad + (-1)^p (\frac{1}{\alpha})^{k-\ell+1}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m-\ell+1)|(I_L)^m[\partial_{x}^{k+1}\phi](x)
	\end{split}
	\end{align*}
 	Now again from the equation in Lemma \ref{lem_D} with using $k-p$ -th sum instead of $k$-th sum, we apply the operator $\mD_L$ to $\mttD_{L}^p[\phi]$:
        \begin{align*}
	\mtD_{L}^{p+1}[\phi](x) & =\mathcal{D}_{L}[\mttD_{L}^{p}][\phi](x)  \\
 & = -\sum_{\ell=1}^{k-p} \left(\frac{1}{\alpha}\right)^{\ell} \left( \partial_{x}^{\ell} \mttD_{L}^{p}[\phi](x) - \partial_{x}^{\ell}\mttD_{L}^{p}[\phi](b) e^{-\alpha(b-x)} \right) -\left(\frac{1}{\alpha}\right)^{k-p+1}I_{L}[\partial_{x}^{k-p+1} \mttD_{L}^{\ell}[\phi]](x) \\
 & = -\sum_{\ell=1}^{k-p} \left(\frac{1}{\alpha}\right)^{\ell} \sum_{m=p+\ell}^{k}C(p,m-\ell)\left(\frac{1}{\alpha}\right)^{m-\ell}  \left(\partial^{m}_{x}\phi(x) -  \partial^{m}_{x}\phi(b) e^{-\alpha(b-x)}\right) \\
 & \quad + (-1)^{p+1} \left(\frac{1}{\alpha}\right)^{k+1} \sum_{\ell=1}^{k-p} \sum\limits_{m = 1}^{p} |C(p-m+1,k-m-\ell+1)|(I_L)^m[\partial_{x}^{k+1}\phi](x)  \\
 & \quad + (-1)^{p+1} \left(\frac{1}{\alpha}\right)^{k+1} \sum\limits_{m = 1}^{p} |C(p-m+1,p-m)|(I_L)^{m+1}[\partial_{x}^{k+1}\phi](x) \\
 & = \sum_{m=p+1}^{k} C(p+1,m)  \left(\frac{1}{\alpha}\right)^{m} \left(\partial^{m}_{x}\phi(x) -  \partial^{m}_{x}\phi(b) e^{-\alpha(b-x)}\right)  \\
 & \quad + (-1)^{p+1} \left(\frac{1}{\alpha}\right)^{k+1} \sum_{m=1}^{p} \left|\sum_{i = p-m+1}^{k-m} C(p-m+1,i) \right| (I_L)^{m}[\partial_{x}^{k+1}\phi](x) + (-1)^{p+1} \left(\frac{1}{\alpha}\right)^{k+1} (I_L)^{p+1}[\partial_{x}^{k+1}\phi](x) \\
 & = \sum_{m=p+1}^{k} C(p+1,m) \left(\frac{1}{\alpha}\right)^{m} \left(\partial^{m}_{x}\phi(x) -  \partial^{m}_{x}\phi(b) e^{-\alpha(b-x)}\right)  \\
 & \quad + (-1)^{p+1} \left(\frac{1}{\alpha}\right)^{k+1} \left( \sum_{m=1}^{p} |C(p-m+2,k-m+1)| (I_L)^{m}[\partial_{x}^{k+1}\phi](x) + (I_L)^{p+1}[\partial_{x}^{k+1}\phi](x) \right)\\
 & = \sum_{m=p+1}^{k} C(p+1,m) \left(\frac{1}{\alpha}\right)^{m} \left(\partial^{m}_{x}\phi(x) -  \partial^{m}_{x}\phi(b) e^{-\alpha(b-x)}\right)  \\
 & \quad + (-1)^{p+1} \left(\frac{1}{\alpha}\right)^{k+1} \left( \sum_{m=1}^{p+1} |C(p-m+2,k-m+1)| (I_L)^{m}[\partial_{x}^{k+1}\phi](x) \right),
	\end{align*}
 which proves \eqref{eqn:DtLAnotherform}.

 Using the format \eqref{eqn:DtLAnotherform}, we see that 
\begin{align*}
 \sum\limits_{p=1}^{k}\mtD_{L}^p[\phi](x) & = -\frac{1}{\alpha}\partial_{x}\phi(x) - \sum_{p=2}^{k} \left(\frac{1}{\alpha}\right)^{p} \left(\partial_{x}^{p}\phi(x) -\partial_{x}^{p}\phi(b) e^{-\alpha(b-x)} \right)- \left(\frac{1}{\alpha}\right)^{k+1}I_{L}[\partial_{x}^{k+1}\phi](x)  \\ 
&  \quad + \sum\limits_{p=2}^{k} \sum_{m=p}^{k}C(p,m)\left(\frac{1}{\alpha}\right)^{m} \left(\partial^{m}_{x}\phi(x) -\partial_{x}^{m}\phi(b) e^{-\alpha(b-x)} \right) \\
& \quad +  \sum\limits_{p=2}^{k} (-1)^p (\frac{1}{\alpha})^{k+1}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m+1)|(I_L)^m[\partial_{x}^{k+1}\phi](x) \\
& = -\frac{1}{\alpha}\partial_{x}\phi(x) + \sum_{p=2}^{k} C_{1,p} \left(\frac{1}{\alpha}\right)^{p} \left(\partial_{x}^{p}\phi(x) -\partial_{x}^{p}\phi(b) e^{-\alpha(b-x)} \right)+  (\frac{1}{\alpha})^{k+1}  \sum\limits_{p=1}^{k} C_{2,p} (I_L)^p[\partial_{x}^{k+1}\phi](x),
\end{align*}
where $C_{1,p}$ and $C_{2,p}$ are two different constants only depending on $p$. This equation proves the case for $k \ge 2$, \eqref{eqn:DtLAnotherform} is a correct approximation of $\phi_x^+$ and so is \eqref{eq:expressionL}. The proof for \eqref{eq:expressionR} is similar to \eqref{eq:expressionL}.
\end{proof}


 \begin{thm}
 Suppose $\phi\in\mathcal{C}^{2k+2}[a,b]$, $k=1, \, 2,\, 3$. Then, the modified partial sums \eqref{eq:mod_sum_0} satisfy
	\begin{align}
		 \|\partial_{xx}\phi(x)-{\mP}^{0}_{k}[\phi](x)\|_{\infty}\leq C \left(\frac{1}{\alpha}\right)^{2k} \|\partial_{x}^{2k+2}\phi(x)\|_{\infty}.
	\end{align}
\end{thm}
%Recalling that we defined $\alpha=\beta/(c\Delta t)$ shows that the modified partial sums \eqref{eq:mod_sum} approximate $\phi_{x}$ with accuracy $\mathcal{O}(\Delta t^k)$.

\begin{proof}
It is obvious for the $k=1$ case from the partial sums \eqref{eq:D0sum} and Lemma \ref{lem_D}. We now consider second derivative approximations, ${\mP}^{0}_{k}[\phi]$, for $k \geq 2$ cases. Similar to the first derivative case, we also give another equivalent definition of $\mtD_{0}^{p}[\phi](x)$ for $2 \le p \le k$ as the follows.  
  \begin{align}\label{eqn:Dt0Anotherform}
  \mtD_{0}^{p}[\phi](x) = & \sum_{m=p}^{k}C(p,m)\left(\frac{1}{\alpha}\right)^{2m} \partial^{2m}_{x}\phi(x) \nonumber \\ 
     & - \frac{1}{2}\sum\limits_{m=p+1}^{k} C(p,m-1) \left( (\frac{1}{\alpha})^{2m} \partial_{x}^{2m}\phi(a) + (-\frac{1}{\alpha})^{2m+1} \partial_{x}^{2m+1}\phi(a)\right) e^{-\alpha(x-a)}
      \nonumber \\ 
     & - \frac{1}{2} \sum\limits_{m=p+1}^{k} C(p,m-1) \left( (\frac{1}{\alpha})^{2m} \partial_{x}^{2m}\phi(b) + (\frac{1}{\alpha})^{2m+1} \partial_{x}^{2m+1}\phi(b)\right) e^{-\alpha(b-x)}  \nonumber\\
 & + (-1)^p (\frac{1}{\alpha})^{2k+2}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m+1)|(I_L)^m[\partial_{x}^{2k+2}\phi](x).
\end{align}
  When $p = 2$, \eqref{eqn:Dt0Anotherform} is same as what we get from \eqref{eq:expression0}. In fact, with \eqref{eqn:Dt0Anotherform}, we have
	\begin{align*}
	\mttD_{0}[\phi](x) = \mtD_{0}[\phi](x) & - \frac{1}{2}\sum\limits_{m=2}^{k} \left( (\frac{1}{\alpha})^{2m} \partial_{x}^{2m}\phi(a) + (-\frac{1}{\alpha})^{2m+1} \partial_{x}^{2m+1}\phi(a)\right) e^{-\alpha(x-a)}
      \\ 
      & - \frac{1}{2} \sum\limits_{m=2}^{k} \left( (\frac{1}{\alpha})^{2m} \partial_{x}^{2m}\phi(b) + (\frac{1}{\alpha})^{2m+1} \partial_{x}^{2m+1}\phi(b)\right) e^{-\alpha(b-x)}.
	\end{align*}
	Then similar to $\mttD_L[\phi](x)$, we can differentiate it,
	\begin{align*}
	\begin{split}
		\partial_{xx} \mttD_0[\phi](x) &= \partial_{xx} \left( -\sum\limits_{p=1}^{k} (\frac{1}{\alpha})^{2p} \partial_{x}^{2p}\phi(x) - (\frac{1}{\alpha})^{2k+2} I_{0}[\partial_{x}^{2k+2}\phi](x) \right) \\
		&=	-\sum\limits_{p=2}^{k} (\frac{1}{\alpha})^{2p-2} \partial_{x}^{2p}\phi(x) - (\frac{1}{\alpha})^{2k} I_{0}[\partial_{x}^{2k+2}\phi](x)
	\end{split}
	\end{align*}
	by using Lemma \ref{lem_D}. Repeating the above process, we can find a general form for $0\leq \ell \leq k$,
	\begin{align*}
		\partial_{x}^{2\ell}\mttD_0[\phi](x) = -\sum\limits_{p=1+\ell}^{k} (\frac{1}{\alpha})^{2p-2\ell} \partial_{x}^{2p}\phi(x) - (\frac{1}{\alpha})^{2k+2-2\ell} I_{0}[\partial_{x}^{2k+2}\phi](x).
	\end{align*}
    Additionally, we need for $0\leq \ell \leq k$,
    \begin{align*}
		\partial_{x}^{2\ell+1}\mttD_0[\phi](x) = -\sum\limits_{p=1+\ell}^{k} (\frac{1}{\alpha})^{2p-2\ell} \partial_{x}^{2p+1}\phi(x) - (\frac{1}{\alpha})^{2k+2-2\ell} \partial_x I_{0}[\partial_{x}^{2k+2}\phi](x),
  % \\
        % \partial_{x}^{2\ell+1}\mttD_0[\phi](a) = -\sum\limits_{p=1+\ell}^{k} (\frac{1}{\alpha})^{2p-2\ell} \partial_{x}^{2p+1}\phi(a) - (\frac{1}{\alpha})^{2k+1-2\ell} I_{0}[\partial_{x}^{2k+2}\phi](a); \\
        % \partial_{x}^{2\ell+1}\mttD_0[\phi](b) = -\sum\limits_{p=1+\ell}^{k} (\frac{1}{\alpha})^{2p-2\ell} \partial_{x}^{2p+1}\phi(b) + (\frac{1}{\alpha})^{2k+1-2\ell} I_{0}[\partial_{x}^{2k+2}\phi](b).
	\end{align*}
    with $\partial_x I_{0}[\partial_{x}^{2k+2}\phi](a) = \alpha I_{0}[\partial_{x}^{2k+2}\phi](a)$ and $\partial_x I_{0}[\partial_{x}^{2k+2}\phi](b) = -\alpha I_{0}[\partial_{x}^{2k+2}\phi](b)$.
	Now again from the equation in Lemma \ref{lem_D} with using $k-1$-th sum instead of $k$-th sum, we apply the operator $\mD_0$ to $\mttD_{0}[\phi]$:
        \begin{align*}
	\mtD_{0}^{2}[\phi](x) & =\mathcal{D}_{0}[\mttD_{0}^{1}][\phi](x)  \\
 & = \sum_{m=2}^{k}(m-1)\left(\frac{1}{\alpha}\right)^{2m} \partial^{2m}_{x}\phi(x) - \frac{1}{2}\sum\limits_{m=3}^{k} (m-2) \left( (\frac{1}{\alpha})^{2m} \partial_{x}^{2m}\phi(a) + (-\frac{1}{\alpha})^{2m+1} \partial_{x}^{2m+1}\phi(a)\right) e^{-\alpha(x-a)}  \\ 
     & \quad - \frac{1}{2} \sum\limits_{m=3}^{k} (m-2) \left( (\frac{1}{\alpha})^{2m} \partial_{x}^{2m}\phi(b) + (\frac{1}{\alpha})^{2m+1} \partial_{x}^{2m+1}\phi(b)\right) e^{-\alpha(b-x)} \\
 & \quad + (\frac{1}{\alpha})^{2k+2} I_0[I_0[\partial_{x}^{2k+2}\phi]](x) + (k-1) (\frac{1}{\alpha})^{2k+2}I_0[\partial_{x}^{2k+2}\phi](x),
	\end{align*}
 which is same as \eqref{eqn:DtLAnotherform} with $p = 2$. 
 Now we prove $p > 2$ cases by induction. Assume that for $p \ge 2$, \eqref{eqn:DtLAnotherform} is equivalent from the definition of \eqref{eq:expressionL}, then we consider $p+1$ case. Since
 \begin{align*}
	\mttD_{0}^{p}[\phi](x)  = & \sum_{m=p}^{k}C(p,m)\left(\frac{1}{\alpha}\right)^{2m} \partial^{2m}_{x}\phi(x) + (-1)^p (\frac{1}{\alpha})^{k+1}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m+1)|(I_0)^m[\partial_{x}^{k+1}\phi](x),
	\end{align*}
 and then we can differentiate it,
 \begin{align*}
	\begin{split}
		\partial_{xx}\mttD_{0}^{p}[\phi](x) &= \partial_{xx} \left( \sum_{m=p}^{k}C(p,m)\left(\frac{1}{\alpha}\right)^{2m} \partial^{2m}_{x}\phi(x) + (-1)^p (\frac{1}{\alpha})^{2k+2}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m+1)|(I_0)^m[\partial_{x}^{2k+2}\phi](x) \right) \\
		&= \sum_{m=p}^{k}C(p,m)\left(\frac{1}{\alpha}\right)^{2m} \partial^{2m+2}_{x}\phi(x) + (-1)^p (\frac{1}{\alpha})^{2k+2}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m+1)| \partial_{xx}(I_0)^m[\partial_{x}^{2k+2}\phi](x)  \\
		&= \sum_{m=p}^{k}C(p,m)\left(\frac{1}{\alpha}\right)^{2m} \partial^{2m+2}_{x}\phi(x) + (-1)^p (\frac{1}{\alpha})^{2k} |C(p,m)|(I_0[\partial_{x}^{2k+2}\phi](x) - \partial_{x}^{2k+2}\phi) \\
        & \quad + (-1)^p (\frac{1}{\alpha})^{2k}  \sum\limits_{m = 2}^{p} |C(p-m+1,k-m+1)|\left((I_0)^m[\partial_{x}^{2k+2}\phi](x) - (I_0)^{m-1}[\partial_{x}^{2k+2}\phi](x)\right) \\ 
        &= \sum_{m=p}^{k-1}C(p,m)\left(\frac{1}{\alpha}\right)^{2m} \partial^{2m+2}_{x}\phi(x) + (-1)^p (\frac{1}{\alpha})^{2k} (I_0)^p [\partial_{x}^{2k+2}\phi](x) \\
        & \quad + (-1)^p (\frac{1}{\alpha})^{2k}  \sum\limits_{m = 1}^{p-1} \left(|C(p-m+1,k-m+1) + C(p-m,k-m)|\right)(I_0)^m[\partial_{x}^{2k+2}\phi](x) \\
        &= \sum_{m=p}^{k-1}C(p,m)\left(\frac{1}{\alpha}\right)^{2m} \partial^{2m+2}_{x}\phi(x) + (-1)^p (\frac{1}{\alpha})^{2k}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m)|(I_0)^m[\partial_{x}^{2k+2}\phi](x),
	\end{split}
	\end{align*}
    where note that if $p$ is even, $|C(p,m)| = C(p,m)$ and if $p$ is odd, $|C(p,m)| = -C(p,m)$. Note that $C(p,m-1) = C(p,m) + C(p-1,m-1)$ and repeating the above process, we can find a general form for $0 \leq \ell \leq k+1-p$, we have   
    \begin{align*}
	\begin{split}
		\partial_{x}^{2\ell} \mttD_{0}^{p}[\phi](x) &= \sum_{m=p}^{k-\ell}C(p,m)\left(\frac{1}{\alpha}\right)^{2m} \partial^{2m+2\ell}_{x}\phi(x) \\  
         & \quad + (-1)^p (\frac{1}{\alpha})^{2k-2\ell+2}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m-\ell+1)|(I_0)^m[\partial_{x}^{2k+2}\phi](x) \\
         & = \sum_{m=p+\ell}^{k}C(p,m-\ell)\left(\frac{1}{\alpha}\right)^{2m-2\ell} \partial^{2m}_{x}\phi(x) \\  
         & \quad + (-1)^p (\frac{1}{\alpha})^{2k-2\ell+2}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m-\ell+1)|(I_0)^m[\partial_{x}^{2k+2}\phi](x).
	\end{split}
	\end{align*}
    Additionally, for $0 \leq \ell \leq k+1-p$, we need:
    \begin{align*}
	\begin{split}
		\partial_{x}^{2\ell+1} \mttD_{0}^{p}[\phi](x) &= 
         \sum_{m=p+\ell}^{k}C(p,m-\ell)\left(\frac{1}{\alpha}\right)^{2m-2\ell} \partial^{2m+1}_{x}\phi(x) \\  
         & \quad + (-1)^p (\frac{1}{\alpha})^{2k-2\ell+2}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m-\ell+1)|\partial_x(I_0)^m[\partial_{x}^{2k+2}\phi](x),
	\end{split}
	\end{align*}
    with $\partial_x(I_0)^m[\partial_{x}^{2k+2}\phi](a) = \alpha (I_0)^m[\partial_{x}^{2k+2}\phi](a)$ and $\partial_x(I_0)^m[\partial_{x}^{2k+2}\phi](b) = -\alpha (I_0)^m[\partial_{x}^{2k+2}\phi](b)$.
 	Now again from the equation in Lemma \ref{lem_D} with using $k-p$ -th sum instead of $k$-th sum, we apply the operator $\mD_0$ to $\mttD_{0}^p[\phi]$:
        \begin{align*}
	\mtD_{0}^{p+1}[\phi](x) & =\mathcal{D}_{0}[\mttD_{0}^{p}][\phi](x)  \\
 & = -\sum\limits_{\ell=1}^{k-p} (\frac{1}{\alpha})^{2\ell} \partial_{x}^{2\ell}\mttD_{0}^{p}[\phi](x) - (\frac{1}{\alpha})^{2k+2-2p} I_{0}[\partial_{x}^{2k+2-2p}\mttD_{0}^{p}[\phi]](x) \\
    & \quad \, + \frac{1}{2}\sum\limits_{\ell=4}^{2k+1-2p} (-\frac{1}{\alpha})^{\ell} \partial_{x}^{\ell}\mttD_{0}^{p}[\phi](a) e^{-\alpha(x-a)}  + \frac{1}{2}\sum\limits_{\ell=4}^{2k+1-2p} (\frac{1}{\alpha})^{\ell} \partial_{x}^{\ell}\mttD_{0}^{p}[\phi](b) e^{-\alpha(b-x)} \\
 & = -\sum_{\ell=1}^{k-p} \sum_{m=p+\ell}^{k}C(p,m-\ell)\left(\frac{1}{\alpha}\right)^{2m} \partial^{2m}_{x}\phi(x) \\
 & \quad + \sum_{\ell=1}^{k-p}\sum\limits_{m = 1}^{p} (-1)^{p+1}  (\frac{1}{\alpha})^{2k+2}   |C(p-m+1,k-m-\ell+1)|(I_0)^m[\partial_{x}^{2k+2}\phi](x) \\
 & \quad + (-1)^{p+1} \left(\frac{1}{\alpha}\right)^{2k+2} \sum\limits_{m = 1}^{p} |C(p-m+1,p-m)|(I_L)^{m+1}[\partial_{x}^{2k+2}\phi](x) \\
 & \quad + \frac{1}{2}\sum_{\ell=2}^{k-p} \sum_{m=p+\ell}^{k}C(p,m-\ell)\left(\frac{1}{\alpha}\right)^{2m} \left( \partial^{2m}_{x}\phi(a)e^{-\alpha(x-a)} + \partial^{2m}_{x}\phi(b)e^{-\alpha(b-x)} \right)\\
 & \quad + \frac{1}{2}\sum_{\ell=2}^{k-p} \sum_{m=p+\ell}^{k}C(p,m-\ell)\left(\frac{1}{\alpha}\right)^{2m} \left( - \partial^{2m}_{x}\phi(a)e^{-\alpha(x-a)} + \partial^{2m}_{x}\phi(b)e^{-\alpha(b-x)} \right)\\
 & = \sum_{m=p+1}^{k} C(p+1,m) \left(\frac{1}{\alpha}\right)^{2m} \partial^{2m}_{x}\phi(x) + (-1)^{p+1} \left(\frac{1}{\alpha}\right)^{2k+2} (I_0)^{p+1}[\partial_{x}^{2k+2}\phi](x)  \\
& \quad + (-1)^{p+1} \left(\frac{1}{\alpha}\right)^{2k+2} \sum_{m=1}^{p} \left|\sum_{i = p-m+1}^{k-m} C(p-m+1,i) \right| (I_0)^{m}[\partial_{x}^{2k+2}\phi](x) \\
 % & \quad + \sum_{\ell=1}^{k-p}\sum\limits_{m = 1}^{p} (-1)^{p+1}  (\frac{1}{\alpha})^{2k+2}   |C(p-m+1,k-m-\ell+1)|(I_0)^m[\partial_{x}^{2k+2}\phi](x) \\
 % & \quad + (-1)^{p+1} \left(\frac{1}{\alpha}\right)^{2k+2} \sum\limits_{m = 1}^{p} |C(p-m+1,p-m)|(I_L)^{m+1}[\partial_{x}^{2k+2}\phi](x) \\
 & \quad - \frac{1}{2} \sum_{m=p+2}^{k} C(p+1,m-1) \left(\frac{1}{\alpha}\right)^{2m} \left( \partial^{2m}_{x}\phi(a)e^{-\alpha(x-a)} + \partial^{2m}_{x}\phi(b)e^{-\alpha(b-x)} \right)\\
 & \quad - \frac{1}{2}\sum_{m=p+2}^{k} C(p+1,m-1) \left(\frac{1}{\alpha}\right)^{2m} \left( - \partial^{2m}_{x}\phi(a)e^{-\alpha(x-a)} + \partial^{2m}_{x}\phi(b)e^{-\alpha(b-x)} \right)\\
 & = \sum_{m=p+1}^{k} C(p+1,m) \left(\frac{1}{\alpha}\right)^{2m} \partial^{2m}_{x}\phi(x)  \\
& \quad + (-1)^{p+1} \left(\frac{1}{\alpha}\right)^{2k+2} \left( \sum_{m=1}^{p+1} |C(p-m+2,k-m+1)| (I_0)^{m}[\partial_{x}^{2k+2}\phi](x) \right)\\
 & \quad - \frac{1}{2} \sum_{m=p+2}^{k} C(p+1,m-1) \left(\frac{1}{\alpha}\right)^{2m} \left( \partial^{2m}_{x}\phi(a)e^{-\alpha(x-a)} + \partial^{2m}_{x}\phi(b)e^{-\alpha(b-x)} \right)\\
 & \quad - \frac{1}{2}\sum_{m=p+2}^{k} C(p+1,m-1) \left(\frac{1}{\alpha}\right)^{2m} \left( - \partial^{2m}_{x}\phi(a)e^{-\alpha(x-a)} + \partial^{2m}_{x}\phi(b)e^{-\alpha(b-x)} \right)\\
\end{align*}
 which proves \eqref{eqn:Dt0Anotherform}.

 Using the format \eqref{eqn:Dt0Anotherform}, we see that 
\begin{align*}
 \sum\limits_{p=1}^{k}\mtD_{0}^p[\phi](x) & = -\frac{1}{\alpha}^2\partial_{xx}\phi(x) -\sum\limits_{p=2}^{k} (\frac{1}{\alpha})^{2p} \partial_{x}^{2p}\phi(x) - (\frac{1}{\alpha})^{2k+2} I_{0}[\partial_{x}^{2k+2}\phi](x) \\
      & \quad + \frac{1}{2}\sum\limits_{p=4}^{2k+1} (-\frac{1}{\alpha})^{p} \partial_{x}^{p}\phi(a) e^{-\alpha(x-a)}
     + \frac{1}{2}\sum\limits_{p=4}^{2k+1} (\frac{1}{\alpha})^{p} \partial_{x}^{p}\phi(b) e^{-\alpha(b-x)} \\
    &  \quad + \sum_{p=2}^{k} \sum_{m=p}^{k}C(p,m)\left(\frac{1}{\alpha}\right)^{2m} \partial^{2m}_{x}\phi(x) \nonumber \\ 
     & - \frac{1}{2}\sum_{p=2}^{k} \sum\limits_{m=p+1}^{k} C(p,m-1) \left( (\frac{1}{\alpha})^{2m} \partial_{x}^{2m}\phi(a) + (-\frac{1}{\alpha})^{2m+1} \partial_{x}^{2m+1}\phi(a)\right) e^{-\alpha(x-a)}
      \nonumber \\ 
     & - \frac{1}{2} \sum_{p=2}^{k} \sum\limits_{m=p+1}^{k} C(p,m-1) \left( (\frac{1}{\alpha})^{2m} \partial_{x}^{2m}\phi(b) + (\frac{1}{\alpha})^{2m+1} \partial_{x}^{2m+1}\phi(b)\right) e^{-\alpha(b-x)}  \nonumber\\
 & + (-1)^p (\frac{1}{\alpha})^{2k+2} \sum_{p=2}^{k} \sum\limits_{m = 1}^{p} |C(p-m+1,k-m+1)|(I_0)^m[\partial_{x}^{2k+2}\phi](x) \\
 & = -\frac{1}{\alpha}^2\partial_{xx}\phi(x) + \sum\limits_{p=2}^{k} C_{1,p} (\frac{1}{\alpha})^{2p} \partial_{x}^{2p}\phi(x) + (\frac{1}{\alpha})^{2k+2} \sum_{m=1}^{k} C_{2,p}(I_0)^m[\partial_{x}^{2k+2}\phi](x) \\
     & + \sum_{m=2}^{k} C_{3,p} \left( (\frac{1}{\alpha})^{2m} \partial_{x}^{2m}\phi(a) + (-\frac{1}{\alpha})^{2m+1} \partial_{x}^{2m+1}\phi(a)\right) e^{-\alpha(x-a)} \\ 
     & + \sum_{m=2}^{k} C_{3,p} \left( (\frac{1}{\alpha})^{2m} \partial_{x}^{2m}\phi(b) + (\frac{1}{\alpha})^{2m+1} \partial_{x}^{2m+1}\phi(b)\right) e^{-\alpha(b-x)}
%  \sum_{p=2}^{k} \left(\frac{1}{\alpha}\right)^{p} \left(\partial_{x}^{p}v(x) -\partial_{x}^{p}v(b) e^{-\alpha(b-x)} \right)- \left(\frac{1}{\alpha}\right)^{k+1}I_{L}[\partial_{x}^{k+1}v](x)  \\ 
% &  \quad + \sum\limits_{p=2}^{k} \sum_{m=p}^{k}C(p,m)\left(\frac{1}{\alpha}\right)^{m} \left(\partial^{m}_{x}\phi(x) -\partial_{x}^{m}\phi(b) e^{-\alpha(b-x)} \right) \\
% & \quad +  \sum\limits_{p=2}^{k} (-1)^p (\frac{1}{\alpha})^{k+1}  \sum\limits_{m = 1}^{p} |C(p-m+1,k-m+1)|(I_L)^m[\partial_{x}^{k+1}\phi](x) \\
% & = -\frac{1}{\alpha}\partial_{x}v(x) + \sum_{p=2}^{k} C_{1,p} \left(\frac{1}{\alpha}\right)^{p} \left(\partial_{x}^{p}v(x) -\partial_{x}^{p}v(b) e^{-\alpha(b-x)} \right)+  (\frac{1}{\alpha})^{k+1}  \sum\limits_{p=1}^{k} C_{2,p} (I_L)^p[\partial_{x}^{k+1}\phi](x),
\end{align*}
where $C_{1,p}$, $C_{2,p}$ and $C_{3,p}$ are three constants only depending on $p$. This equation proves the case for $k \ge 2$, \eqref{eqn:Dt0Anotherform} is a correct approximation of $\phi_{xx}$ and so is \eqref{eq:expression0}. 








% (2) Let 
% \begin{align*}
%     \tI_0[v](x) =  I_{0}[v](x) & + \frac{\mu I_{0}[v](a)-I_{0}[v](b)}{1-\mu^2} e^{-\alpha(b-x)} + \frac{\mu I_{0}[v](b)-I_{0}[v](a)}{1-\mu^2} e^{-\alpha(x-a)}.
% \end{align*}
% Since $\partial_{xx}I_{0}[v](x) = \alpha^2(I_{0}[v](x) - v)$, we have 
% \begin{align}\label{eqn:tI0relation}
%     \partial_{xx} \tI_0[v](x) & =\partial_{xx}I_{0}[v](x) + \alpha^2 (\frac{\mu I_{0}[v](a)-I_{0}[v](b)}{1-\mu^2} e^{-\alpha(b-x)} + \frac{\mu I_{0}[v](b)-I_{0}[v](a)}{1-\mu^2} e^{-\alpha(x-a)}) \nonumber \\ 
%     & = \alpha^2(\tI_{0}[v](x) - v). 
% \end{align}
% And what we left is to follow the same procedure as (1) to prove the result. 
	% where $Q_{2}(x)=(k-2)\mathcal{L}^{-1}_{0}[\partial^{2k+2}_{x}v](x) + \left(\mathcal{L}^{-1}_{0}\right)^2[\partial^{2k+2}_{x}v](x)$. Repeating the process, and finally, we arrive at
	% $$\sum_{p=1}^{k}\mathcal{D}^{p}_{0}[v](x)=-\frac{1}{\alpha^2}\partial_{xx}v(x) + \left(\frac{1}{\alpha}\right)^{2k+2} Q_{k}(x),$$
	% where $Q_{k}(x)$ is a linear combination of functions $\left(\mathcal{L}^{-1}_{0}\right)^{p}[\partial^{2k+2}_{x}v](x)$, $p=1,2,\ldots,k$. Note that, for any $w(x)\in\mathit{C}[a,b]$, we have
	% $$\|\mathcal{L}^{-1}_{0}[w](x)\|_{\infty}\leq C_{0} \|w\|_{\infty},$$
	% where $C_{0}$ is a constant independent of $w$ and $\alpha$. Then, there is a constant $C$ only depending on $k$, such that
	% $$\|\partial_{xx}v(x)+\alpha^2\sum_{p=1}^{k}\mathcal{D}^{p}_{0}[v](x)\|_{\infty}=\|\left(\frac{1}{\alpha}\right)^{2k}Q_{k}(x)\|_{\infty}\leq C\left(\frac{1}{\alpha}\right)^{2k} \|\partial_{x}^{2k+2}v(x)\|_{\infty},$$
	% which completes the proof.
\end{proof}



